UIT-ViCoV19QA: A Dataset for COVID-19 Community-based Question Answering on Vietnamese Language

For the last two years, from 2020 to 2021, COVID-19 has broken disease prevention measures in many countries, including Vietnam, and negatively impacted various aspects of human life and the social community. Besides, the misleading information in the community and fake news about the pandemic are also serious situations. Therefore, we present the first Vietnamese community-based question answering dataset for developing question answering systems for COVID-19 called UIT-ViCoV19QA. The dataset comprises 4,500 question-answer pairs collected from trusted medical sources, with at least one answer and at most four unique paraphrased answers per question. Along with the dataset, we set up various deep learning models as baseline to assess the quality of our dataset and initiate the benchmark results for further research through commonly used metrics such as BLEU, METEOR, and ROUGE-L. We also illustrate the positive effects of having multiple paraphrased answers experimented on these models, especially on Transformer - a dominant architecture in the field of study.

==> old/sections/1-intro1.tex <==
\section{Introduction}

Community-based Question answering (CQA) is a task of question answering based on the wisdom of the crowd \cite{zhang2021graph}. In CQA, information seekers post their questions on a public website or forum, and other users answer them. This kind of question-answering behavior is popular in people's daily lives. For example, Quora\footnote{\url{https://www.quora.com/}} and Reddit\footnote{\url{https://www.reddit.com/}} are several large forums for question-answering. The CQA enables people to ask and answer questions easily \cite{qiu2015convolutional}. Additionally, the development of question and answering systems means computers can now understand and answer the questions of users. 

In Vietnam, the year from 2020 to 2021 witnessed the COVID-19 pandemic. Information about the COVID-19 spreading situation, medical care, self-quarantine, vaccination policies, and regulations by the government to prevent the spread of COVID-19 are essential to citizens. People frequently ask questions about the COVID-19 situation, what to do when contacting COVID-19 patients, the vaccination policies, and more. This is our motivation to construct a dataset 
% for the question and answering dataset 
to help build a question answering system based on CQA about COVID-19 in Vietnamese. Apart from the dataset, we also propose various baseline models to evaluate our dataset's quality. Our paper has three main contributions:

\begin{enumerate}
  \item We introduce ViCovidQA, a collection of 4,500 question-answer pairs about the COVID-19 pandemic constructed from trusted sources and the first community-based question answering dataset about COVID-19 for Vietnamese. From the initial response, we perform a paraphrasing process to create up to three more unique paraphrased answers. 
  \item We experiment with various Sequence-to-Sequence baselines to assess our quality of the dataset and establish a future research benchmark.
  \item We illustrate that models trained on multiple paraphrased answers tend to have better generalization than those trained using only one answer. This reflects the advantage of having multiple paraphrased answers in single-turn conversational question answering.
\end{enumerate}

The rest of this paper is structured as follows. In the following section, we review the related works. In Section 3, we describe the dataset in detail and its statistics. Section 4 is devoted to methodologies and experiments configurations. The results and benchmarks are described in Section 5. Finally, we conclude and present future works in Section 6.

==> old/sections/2-related1.tex <==
\section{Related works}
Question answering systems consist of the single-turn and multi-turn QA. According to \cite{del2021question}, the single-turn QA takes the questions as input and returns the output without context. Single-turn QA includes Text-based QA (SQuAD \cite{rajpurkar-etal-2016-squad}, RACE \cite{lai-etal-2017-race}),
Visual-QA (VQA \cite{goyal2017making}), Community-based QA (ANTIQUE \cite{hashemi2020antique}), and Knowledge-based QA (MetaQA \cite{zhang2018variational}) In contrast, the multi-turn QA take the questions as input belong with contexts such as conversation history, which is called the Conversational QA (CoQA \cite{reddy-etal-2019-coqa}, QuAC \cite{choi-etal-2018-quac}). Additionally, to verbalize the response from the question, the ParaQA dataset \cite{kacupaj2021paraqa} used the paraphrasing techniques. Each question in the ParaQA dataset has at least two more answers. In particular, some questions contain eight responses.

On the other hand, many efforts to create the question answering corpora in Vietnamese such as UIT-ViQuAD \cite{nguyen2020vietnamese}, UIT-ViNewsQA \cite{van2020new}, ViMMRC \cite{van2020enhancing} for text-based question answering, ViVQA \cite{tran2021vivqa} for visual-based QA, and ViCoQA \cite{luu2021conversational} for conversational QA. Our works contributes to the corpora for Vietnamese as Community-based QA dataset. With the idea from the ParaQA dataset \cite{kacupaj2021paraqa}, we create up to three responses from initial answer for each question
%at least two responses for each question
in our dataset to make the dataset verbalized. 

==> old/sections/3-dataset1.tex <==
\section{Dataset} In order to publish a high-quality dataset for the research community and be able to experiment with the baseline models, we have investigated building a dataset for Vietnamese, a low-resource language in the field of study. This section describes the construction of  ViCovidQA in detail and presents some statistics from the dataset. The overview of the dataset construction workflow is illustrated in Figure \ref{fig_workflow}.


\begin{figure*}[ht]
\centering
\includegraphics[width=.9\textwidth]{figures/workflow.png}
\caption{An overview of ViCovidQA constructing workflow}
\label{fig_workflow}
\end{figure*}

\subsection{Data Collection}
%[COVID-19 la chu de nong hoi, song song do la bung no tin gia ...].
We choose question-answer pairs from FAQ documents that are publicly available on websites of respected health care organizations in Vietnam and overseas, including The Centers for Disease Control and Prevention (CDC), United Nations Children's Fund (UNICEF), The Ministry of Health of Vietnam, Vietnam Government Portal and other trusted medical institutions. Each web page provides different topics about the COVID-19 pandemic compiled in Vietnamese and often includes similar information extracted during the crawl. The following topics are covered in our dataset: origin, outbreak, and name of the disease; spread; symptoms; prevention, treatment guidelines, and nutrition; treatment models; variants of COVID-19; vaccines and vaccination; moving between areas, entry, and travel; isolation, quarantine, lockdown and social distancing; policies and sanctions; financial support; post-COVID-19; COVID-19 in children. Disease statistics in Vietnam and worldwide are not included in our dataset.

Next, we develop handcrafted patterns for each website to automatically extract question-answer pairs based on the document structure, typically in HTML and PDF format. Throughout the collecting phase, we maintain the length of both question and answer to retain information. Therefore, the collected content could be a sentence, a paragraph, or a passage determined by the author or compiler. This poses a tremendous challenge for Sequence-to-Sequence models to produce good results, which makes it an ideal material for further investigations.

\subsection{Data Pre-processing}
A two-stage pre-processing is performed on the collected question-answer pairs. First, we detect duplicate pairs using Cosine similarity at the collection-level and consider taking them out of the collection. During the crawl, we also try to identify and remove pairs that have inappropriate content, such as articles that are neither related to COVID-19 nor the Vietnamese community or too complicated to comprehend. Some examples are shown in Table \ref{tbl_examples} to illustrate the questions of irrelevant pairs.

Second, at the pair-level, we check the spelling and correct mistakes. Undesirable artifacts, erroneous character and HTML tags will also be removed in this stage. In case the collected articles are too long or contains more than three paragraphs, extracted answers will be manually reduced in length by removing unnecessary information, such as source name, footnote, greetings, preliminary, over-specified explanations, and farewell. After this step, 4,500 Vietnamese question-answer pairs about  COVID-19 are achieved from trusted FAQ sources. Some examples of the collected question-answer pairs are also shown in Table \ref{tbl_examples}.

% \begin{table*}[ht]
% \begin{center}
% \begin{tabular}{p{0.95\linewidth}}
% \hline \textbf{\underline{Question:}} Có những nguồn lực nào dành cho vấn đề mai táng cựu chiến binh là Người Mỹ Da Đỏ/Người Alaska Bản Địa? (\textbf{English:} What resources are available for American Indian/Alaska Native veteran burial?)\\

% \textbf{\underline{Answer:}} Vợ/chồng và gia đình Cựu Chiến Binh Người Mỹ Da Đỏ/Người Alaska Bản Địa có thể đủ điều kiện được hỗ trợ mai táng. Quyền lợi chôn cất có thể gồm khai huyệt và an táng, chăm sóc phần mộ vĩnh viễn, bia hoặc dấu tưởng niệm của chính phủ, cờ tang và Chứng Nhận của Tổng Thống, hoàn toàn miễn phí cho gia đình. Một số cựu chiến binh cũng có thể đủ điều kiện nhận tiền để giúp đài thọ chi phí (phụ cấp chôn cất). (\textbf{English:} Spouses and families of American Indian/Alaska Native Veterans may be eligible for burial assistance. Burial benefits may include burial and burial, permanent grave care, government memorials or markers, mourning flags and Presidential Certificates, all at no cost to the family. Some veterans may also qualify for money to help cover expenses (burial allowance).\\
%  \hline

% \textbf{\underline{Question:}} Mất bao lâu để hòa tan hàm lượng các loại hạt tạp gây lây nhiễm trong một căn phòng sau khi chúng được tạo ra? (How long does it take to dissolve infectious impurities in a room after they are created?)\\

% \textbf{\underline{Answer:}} Khi những giọt nước lớn (từ 100 micrometer [µm] trở lên) sẽ lắng xuống các bề mặt xung quanh trong vài giây, những hạt nhỏ hơn có thể ngưng đọng trong không khí lâu hơn. Có thể mất vài phút để các hạt có kích thước 10 µm lắng xuống, trong lúc các hạt có kích thước từ 5 µm trở xuống có thể không lắng xuống trong nhiều giờ hoặc nhiều ngày. ... ( \textbf{English:}
% As large water droplets (100 micrometers [µm] or more) settle on surrounding surfaces in seconds, the smaller particles can remain airborne for longer. It can take several minutes for particles 10 µm in size to settle, while particles 5 µm in size or less may not settle for hours or days. ... )\\\hline


% \end{tabular}
% \end{center}
% \caption{Examples of question-answer pairs that have inappropriate content or too complicated}
% \label{tbl_example_wrongs} 
% \end{table*}


\begin{table*}[ht]
\renewcommand{\arraystretch}{1.2}
\begin{center}
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{\underline{Inappropriate questions:}}\\
1. Có những nguồn lực nào dành cho vấn đề mai táng cựu chiến binh là Người Mỹ Da Đỏ/Người Alaska Bản Địa? [\textbf{English: }What resources are available for American Indian/Alaska Native veteran burial?]\\
2. Mất bao lâu để hòa tan hàm lượng các loại hạt tạp gây lây nhiễm trong một căn phòng sau khi chúng được tạo ra? [\textbf{English: }How long does it take to dissolve infectious impurities in a room after they are created?]\\
3. "Luồng không khí có định hướng" nghĩa là gì? Nên sử dụng như thế nào và ở đâu? [\textbf{English: }What is meant by “directional airflow?” How and where should it be used?]\\


\toprule
\toprule
\textbf{\underline{Relevant question-answer pairs:}}\\
\textbf{Question:} Xử lý triệu chứng ho khi chăm sóc F0 tại nhà thế nào? [\textbf{English: }How to handle cough symptoms when taking care of F0 patient at home?]\\
\textbf{Answer:} Dùng thuốc giảm ho theo đơn của bác sĩ. Có thể dùng thêm các vitamin theo đơn thuốc của bác sĩ. [\textbf{English: }Take cough suppressants as prescribed by your doctor. Additional vitamins can be taken according to the doctor's prescription.]\\ 
\midrule
\textbf{Question:} Tôi đang điều trị viêm tiết niệu và viêm dạ dày hội chứng ruột kích thích thì có tiêm vaccine Covid-19 được hay không? [\textbf{English: }I am being treated for UTIs and gastritis with irritable bowel syndrome, can I get the Covid-19 vaccine?]\\
\textbf{Answer:} Với bệnh cấp tính mà anh/chị đang mắc phải cần được điều trị ổn định trước, sức khỏe tốt, bình thường thì có thể tiêm vaccine Covid-19. [\textbf{English: }If you have an acute illness that are stably treated, if you are in good health, you can receive the Covid-19 vaccine.]\\
\midrule
\textbf{Question:} Hỗ trợ hô hấp cho trẻ em nhiễm COVID-19 ở thế nặng như thế nào? [\textbf{English: }How to provide respiratory support to children with COVID-19 in severe condition?]\\
\textbf{Answer:} Thở mask có túi Hoặc: NCPAP, HPNO, NIPPV [\textbf{English: }Apply breathing mask with bag or: NCPAP, HPNO, NIPPV]\\\toprule
\end{tabular}
\end{center}
\caption{Examples of irrelevant questions that were removed and question-answer pairs from ViCovidQA}
\label{tbl_examples} 
\end{table*}


% \begin{table*}[ht]
% \begin{center}
% \begin{tabular}{|p{0.3\linewidth}|p{0.6\linewidth}|}
% \hline \bf Question & \bf Answer \\ \hline
% \textbf{Vietnamese:} Có những nguồn lực nào dành cho vấn đề mai táng cựu chiến binh là Người Mỹ Da Đỏ/Người Alaska Bản Địa? & \textbf{Vietnamese:} Vợ/chồng và gia đình Cựu Chiến Binh Người Mỹ Da Đỏ/Người Alaska Bản Địa có thể đủ điều kiện được hỗ trợ mai táng. Quyền lợi chôn cất có thể gồm khai huyệt và an táng, chăm sóc phần mộ vĩnh viễn, bia hoặc dấu tưởng niệm của chính phủ, cờ tang và Chứng Nhận của Tổng Thống, hoàn toàn miễn phí cho gia đình. Một số cựu chiến binh cũng có thể đủ điều kiện nhận tiền để giúp đài thọ chi phí (phụ cấp chôn cất).\\


% \textbf{English:} What resources are available for American Indian/Alaska Native veteran burial? &\textbf{English:} Spouses and families of American Indian/Alaska Native Veterans may be eligible for burial assistance. Burial benefits may include burial and burial, permanent grave care, government memorials or markers, mourning flags and Presidential Certificates, all at no cost to the family. Some veterans may also qualify for money to help cover expenses (burial allowance).\\ \hline

% \textbf{Vietnamese:} Mất bao lâu để hòa tan hàm lượng các loại hạt tạp gây lây nhiễm trong một căn phòng sau khi chúng được tạo ra? 

% & \textbf{Vietnamese:} Khi những giọt nước lớn (từ 100 micrometer [µm] trở lên) sẽ lắng xuống các bề mặt xung quanh trong vài giây, những hạt nhỏ hơn có thể ngưng đọng trong không khí lâu hơn. Có thể mất vài phút để các hạt có kích thước 10 µm lắng xuống, trong lúc các hạt có kích thước từ 5 µm trở xuống có thể không lắng xuống trong nhiều giờ hoặc nhiều ngày. ...\\


% \textbf{English:} How long does it take to dissolve infectious impurities in a room after they are created? & \textbf{English:} As large water droplets (100 micrometers [µm] or more) settle on surrounding surfaces in seconds, the smaller particles can remain airborne for longer. It can take several minutes for particles 10 µm in size to settle, while particles 5 µm in size or less may not settle for hours or days. ... \\
% \hline
% \end{tabular}
% \end{center}
% \caption{\label{font-table} Examples of question-answer pairs that have inappropriate content or too complicated}
% \end{table*}

% \subsubsection{Question Types}
\subsection{Paraphrase Generation Process}
Inspired by the concept of \newcite{kacupaj2021paraqa}, we have investigated extending our dataset using the following paraphrasing methods on Vietnamese samples:

\begin{itemize}
    \item Rearrange words, phrases, or sentences in the initial answer to create new responses without changing their meaning.
    \item Reduce or diversify the content of the initial answer.
    \item Paraphrase the initial answer using synonyms and similar structures.
\end{itemize}

We apply these methods to manually create up to three individual paraphrased responses consecutively for each question-answer pair. Newly created answers will be annotated in order to indicate the minimum number of answers per question.

After creating multiple paraphrased versions of the initial answer, we perform a cross-checking process to correct the spelling mistakes and grammatical errors as well as modify and rephrase digressive answers. By the end of this phase, the ViCovidQA dataset is entirely constructed with 4,500 question-answer pairs containing at least one answer and at most four unique paraphrased answers per question.

\subsection{Statistics}
The statistics of the training, development, and test sets are described in Table \ref{tbl_stat_dataset}. The ViCovidQA dataset consists of 4,500 question-answer pairs in total. In the table, the average length, as well as the vocabulary size \footnote{We use underthesea package: \url{https://github.com/undertheseanlp/underthesea} for word segmentation.} of questions and answers, are also presented.

Figure \ref{fig_distribute_response} illustrates the distribution of 4,500 questions of ViCovidQA based on number of answers per question. The figure shows that the dataset contains 1800 questions that have at least two answers, 700 questions have at least three answers and half of them have a maximum of four paraphrased answers.

\begin{figure}[ht]
\centering
\hspace*{-0.6cm}\includegraphics[width=0.5
\textwidth]{figures/dist.png}
\setlength{\belowcaptionskip}{-10pt}
\caption{Distribution of total number of answers per question in ViCovidQA}
\label{fig_distribute_response}
\end{figure}


\begin{table*}[ht]
\centering
\begin{tabular}{@{}llrrrr@{}}
\toprule
\multicolumn{2}{l}{}                                                               & \multicolumn{1}{c}{\textbf{Train}}        & \multicolumn{1}{c}{\textbf{Dev.}}         & \multicolumn{1}{c}{\textbf{Test}}        & \multicolumn{1}{c}{\textbf{All}}          \\ \midrule
{\color[HTML]{000000} }                           & Number of question-answer pairs & 3500                             & 500                             & 500                             & 4500                             \\
{\color[HTML]{000000} }                           & Average question length        & \cellcolor[HTML]{FFFFFF}31.44   & \cellcolor[HTML]{FFFFFF}33.66   & \cellcolor[HTML]{FFFFFF}32.32  & \cellcolor[HTML]{FFFFFF}31.79  \\
{\color[HTML]{000000} }                           & Average answer length          & \cellcolor[HTML]{FFFFFF}120.53 & \cellcolor[HTML]{FFFFFF}116.04 & \cellcolor[HTML]{FFFFFF}118.11 & \cellcolor[HTML]{FFFFFF}119.76 \\
{\color[HTML]{000000} }                           & Question vocabulary size       & \cellcolor[HTML]{FFFFFF}4396     & \cellcolor[HTML]{FFFFFF}1869    & \cellcolor[HTML]{FFFFFF}1770    & \cellcolor[HTML]{FFFFFF}4924     \\
\multirow{-5}{*}{{\color[HTML]{000000} \textbf{Answer 1}}} & Answer vocabulary size         & \cellcolor[HTML]{FFFFFF}8537     & \cellcolor[HTML]{FFFFFF}3689    & \cellcolor[HTML]{FFFFFF}3367    & \cellcolor[HTML]{FFFFFF}9411     \\\midrule
{\color[HTML]{000000} }                           & Number of question-answer pairs & \cellcolor[HTML]{FFFFFF}1390     & 209                             & 201                             & 1800                             \\
{\color[HTML]{000000} }                           & Average question length        & \cellcolor[HTML]{FFFFFF}35.56  & \cellcolor[HTML]{FFFFFF}39.22 & \cellcolor[HTML]{FFFFFF}39.72 & \cellcolor[HTML]{FFFFFF}36.45  \\
{\color[HTML]{000000} }                           & Average answer length          & \cellcolor[HTML]{FFFFFF}40.54   & \cellcolor[HTML]{FFFFFF}39.25 & \cellcolor[HTML]{FFFFFF}42.73 & \cellcolor[HTML]{FFFFFF}40.64  \\
{\color[HTML]{000000} }                           & Question vocabulary size       & \cellcolor[HTML]{FFFFFF}2883     & \cellcolor[HTML]{FFFFFF}1269    & \cellcolor[HTML]{FFFFFF}1207    & \cellcolor[HTML]{FFFFFF}3305     \\
\multirow{-5}{*}{{\color[HTML]{000000} \textbf{Answer 2}}} & Answer vocabulary size         & \cellcolor[HTML]{FFFFFF}2632     & \cellcolor[HTML]{FFFFFF}1098    & \cellcolor[HTML]{FFFFFF}1129    & \cellcolor[HTML]{FFFFFF}2949     \\\midrule
{\color[HTML]{000000} }                           & Number of question-answer pairs & 542                              & 79                              & 79                              & 700                              \\
{\color[HTML]{000000} }                           & Average question length        & \cellcolor[HTML]{FFFFFF}34.77  & \cellcolor[HTML]{FFFFFF}36.70 & \cellcolor[HTML]{FFFFFF}39.28 & \cellcolor[HTML]{FFFFFF}35.49  \\
{\color[HTML]{000000} }                           & Average answer length          & \cellcolor[HTML]{FFFFFF}28.68  & \cellcolor[HTML]{FFFFFF}26.43 & \cellcolor[HTML]{FFFFFF}30.89 & \cellcolor[HTML]{FFFFFF}28.67  \\
{\color[HTML]{000000} }                           & Question vocabulary size       & \cellcolor[HTML]{FFFFFF}1836     & \cellcolor[HTML]{FFFFFF}717     & \cellcolor[HTML]{FFFFFF}693     & \cellcolor[HTML]{FFFFFF}2111     \\
\multirow{-5}{*}{{\color[HTML]{000000} \textbf{Answer 3}}} & Answer vocabulary size         & \cellcolor[HTML]{FFFFFF}1554     & \cellcolor[HTML]{FFFFFF}503     & \cellcolor[HTML]{FFFFFF}585     & \cellcolor[HTML]{FFFFFF}1753     \\\midrule
{\color[HTML]{000000} }                           & Number of question-answer pairs & 272                              & 39                              & 39                              & 350                              \\
{\color[HTML]{000000} }                           & Average question length        & \cellcolor[HTML]{FFFFFF}36.57  & \cellcolor[HTML]{FFFFFF}37.59 & \cellcolor[HTML]{FFFFFF}42.15 & \cellcolor[HTML]{FFFFFF}37.10  \\
{\color[HTML]{000000} }                           & Average answer length          & \cellcolor[HTML]{FFFFFF}29.75  & \cellcolor[HTML]{FFFFFF}29.03 & \cellcolor[HTML]{FFFFFF}35.72 & \cellcolor[HTML]{FFFFFF}30.25  \\
{\color[HTML]{000000} }                           & Question vocabulary size       & \cellcolor[HTML]{FFFFFF}1315     & \cellcolor[HTML]{FFFFFF}470     & \cellcolor[HTML]{FFFFFF}460     & \cellcolor[HTML]{FFFFFF}1519     \\
\multirow{-5}{*}{{\color[HTML]{000000} \textbf{Answer 4}}} & Answer vocabulary size         & \cellcolor[HTML]{FFFFFF}924      & \cellcolor[HTML]{FFFFFF}353     & \cellcolor[HTML]{FFFFFF}374     & \cellcolor[HTML]{FFFFFF}1075     \\ \midrule
\end{tabular}
\caption{Overall statistics of the ViCovidQA dataset.}
\label{tbl_stat_dataset}
\end{table*}


==> old/sections/4-method1.tex <==
\section{Methodologies}

\subsection{Baseline Models}
% [Kể từ sự xuất hiện của Transformer, cùng với các mô hình RNN dùng cơ chế attention ma kết quả state of the art da dat duoc tren tac vu hỏi đáp, bài toán dịch máy, text sumarization.]
This experimental section set up various deep learning models with Encoder-Decoder architecture to evaluate the ViCovidQA dataset. These models have achieved significant results on many sequence-to-sequence learning tasks that involve long sequences, such as machine translation, text summarization, and question answering.

\begin{itemize}
    
    \item \textbf{Attention-based Recurrent Neural Network}: We implement recurrent neural network (RNN) models with two attention mechanism - Bahdanau Attention \cite{bahdanau2016neural} and Luong Attention \cite{luong-etal-2015-effective}. To ensure that the results are comparable, we set up these models with similar hyperparameters in the encoder and decoder as follows: an embedding layer with dimension 512, two hidden layers of 512 gated recurrent unit (GRU) cells, and a drop-out rate of 0.5. Bidirectional GRU (Bi-GRU) is applied in the encoder of both models to help them understand the context better. For simplicity, we annotate RNN models using Bahdanau attention and Luong Attention as RNN-1 and RNN-2, respectively.
    
    \item \textbf{Convolutional} \cite{10.5555/3305381.3305510}:
    Different from RNN, convolutional neural network uses many convolutional layers typically applied in image processing. Each layer uses filters to learn to extract different features from the text. In our experiments, the hyperparameters of models are set as follows: embedding layer with dimension 512, three convolutional layers with hidden size 512 use 1024 filters with kernel size 3 x 3, and drop-out probability 0.5.
     
    \item \textbf{Transformer} \cite{NIPS2017_3f5ee243}: As a dominant architecture in natural language processing (NLP), the model and its variants, such as BERT and pre-trained versions of BERT, have been commonly used to achieve state-of-the-art results for many tasks in the field. We set up the Transformer with these settings: embedding layer with dimension 512, two layers with 8 self-attention heads, positional embedding layer with max length 500, position-wise feed-forward layer with dimension 2048 and  drop-out rate 0.5.
    \end{itemize}


\subsection{Evaluation Metrics}
We utilize three standard metrics for evaluating baseline models. These metrics are commonly used in machine translation and text summarization tasks to compare the generated text with human performance.
\begin{itemize}
    \item \textbf{BLEU} \cite{papineni2002bleu}: BLEU is an n-gram based evaluation metric, widely used for Machine Translation (MT) evaluation to claim a high correlation with human judgments of quality. It aims to count the n-gram overlaps in the reference by taking the maximum count of each n-gram and clipping the count of the n-grams in the candidate text to the maximum count in the reference. In our experiments, BLEU score is calculated using unigram (BLEU-1) and 4-gram (BLEU-4) with uniform weight $w_n=0.25$.
    
    \item \textbf{METEOR} \cite{lavie-agarwal-2007-meteor}: The metric is based on the harmonic mean of unigram precision and recall, with recall weighted higher than precision. Moreover, it has several features not found in other metrics, such as stemming and synonymy matching, along with the standard exact word matching. Unfortunately, those features are not yet supported for the Vietnamese language. We set up standard METEOR only using exact matching for evaluation with $\alpha = 0.9$, $\beta = 3.0$ and $\gamma = 0.5$.
    \item \textbf{ROUGE-L} \cite{lin-2004-rouge}: This metric measures the longest common subsequence (LCS) between our model output and reference. The idea here is that a longer shared sequence would indicate more similarity between the two sequences. An advantage of using LCS is that it does not require consecutive matches but in-sequence matches that reflect sentence-level word order. For each generated answer, we choose the best score achieved from comparing it with all existing reference answers.
    % Since it automatically includes longest in-sequence common n-grams, you don’t need a predefined n-gram length.
\end{itemize}

% In our experiments, we use 
% BLEU metric and METEOR metric are commonly used in machine translation task to evaluate model performance to compare predicted text with human translation. 

\subsection{Experimental Configuration}


\begin{table*}[ht]
\setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1}
\small
\centering
\begin{tabular}{l|l|ccccc}
\toprule
\multicolumn{2}{c}{{\color[HTML]{000000} \textbf{Model}}} &
  {\color[HTML]{000000} \textbf{\# answers}} &
  {\color[HTML]{000000} \textbf{BLEU-1 (\%)}} &
  {\color[HTML]{000000} \textbf{BLEU-4 (\%)}} &
  {\color[HTML]{000000} \textbf{METEOR (\%)}} &
  {\color[HTML]{000000} \textbf{ROUGE-L (\%)}} \\\midrule
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 1} &
  {\color[HTML]{000000} 21.79} &
  {\color[HTML]{000000} 10.29} &
  {\color[HTML]{000000} 25.34} &
  {\color[HTML]{000000} 32.36} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 2} &
  {\color[HTML]{000000} \textbf{\underline{26.62}}} &
  {\color[HTML]{000000} \textbf{12.86}} &
  {\color[HTML]{000000} 25.15} &
  {\color[HTML]{000000} 33.66} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 3} &
  {\color[HTML]{000000} 26.09} &
  {\color[HTML]{000000} 12.63} &
  {\color[HTML]{000000} \textbf{\underline{25.98}}} &
  {\color[HTML]{000000} \textbf{33.68}} \\
\multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} RNN-1 \cite{bahdanau2016neural}}}} &
  {\color[HTML]{000000} 4} &
  {\color[HTML]{000000} 24.56} &
  {\color[HTML]{000000} 12.27} &
  {\color[HTML]{000000} 23.91} &
  {\color[HTML]{000000} 32.57} \\\midrule
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 1} &
  {\color[HTML]{000000} 21.04} &
  {\color[HTML]{000000} 10.94} &
  {\color[HTML]{000000} \textbf{24.72}} &
  {\color[HTML]{000000} \textbf{\underline{33.95}}} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 2} &
  {\color[HTML]{000000} 24.07} &
  {\color[HTML]{000000} 11.30} &
  {\color[HTML]{000000} 23.81} &
  {\color[HTML]{000000} 31.92} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 3} &
  {\color[HTML]{000000} 23.8} &
  {\color[HTML]{000000} 10.95} &
  {\color[HTML]{000000} 23.65} &
  {\color[HTML]{000000} 31.65} \\
\multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} RNN-2 \cite{luong-etal-2015-effective}}}} &
  {\color[HTML]{000000} 4} &
  {\color[HTML]{000000} \textbf{24.38}} &
  {\color[HTML]{000000} \textbf{12.30}} &
  {\color[HTML]{000000} 24.29} &
  {\color[HTML]{000000} 32.09} \\\midrule

\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 1} &
  {\color[HTML]{000000} 19.17} &
  {\color[HTML]{000000} 9.51} &
  {\color[HTML]{000000} \textbf{22.76}} &
  {\color[HTML]{000000} \textbf{32.29}} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 2} &
  {\color[HTML]{000000} 21.63} &
  {\color[HTML]{000000} 10.81} &
  {\color[HTML]{000000} 20.66} &
  {\color[HTML]{000000} 30.71} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 3} &
  {\color[HTML]{000000} 22.08} &
  {\color[HTML]{000000} 10.68} &
  {\color[HTML]{000000} 20.96} &
  {\color[HTML]{000000} 30.84} \\
\multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} Convolutional \cite{10.5555/3305381.3305510}}}} &
  {\color[HTML]{000000} 4} &
  {\color[HTML]{000000} \textbf{23.26}} &
  {\color[HTML]{000000} \textbf{10.93}} &
  {\color[HTML]{000000} 21.84} &
  {\color[HTML]{000000} 31.15} \\\midrule
 
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 1} &
  {\color[HTML]{000000} 21.84} &
  {\color[HTML]{000000} 10.82} &
  {\color[HTML]{000000} 23.37} &
  {\color[HTML]{000000} 31.67} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 2} &
  {\color[HTML]{000000} 24.81} &
  {\color[HTML]{000000} 13.22} &
  {\color[HTML]{000000} \textbf{24.60}} &
  {\color[HTML]{000000} \textbf{32.25}} \\
\multicolumn{2}{l}{{\color[HTML]{000000} }} &
  {\color[HTML]{000000} 3} &
  {\color[HTML]{000000} 24.90} &
  {\color[HTML]{000000} 13.64} &
  {\color[HTML]{000000} 21.72} &
  {\color[HTML]{000000} 32.20} \\
\multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} Transformer \cite{NIPS2017_3f5ee243}}}} &
  {\color[HTML]{000000} 4} &
  {\color[HTML]{000000} \textbf{25.19}} &
  {\color[HTML]{000000} \textbf{\underline{14.38}}} &
  {\color[HTML]{000000} 23.11} &
  {\color[HTML]{000000} 32.19} \\\midrule

\end{tabular}
\caption{Performance of baseline models on different dataset settings}
\label{tbl_overall_results}
\end{table*}

To illustrate the benefit of having multiple paraphrased answer, we conduct and run individual experiment with four different dataset settings: one answer, two answers, three answers and finally, four paraphrased answers per question.

For Transformer, we implement Adam optimizer with parameters as follows: $\beta_1=0.9$, $\beta_2=0.98$, $\epsilon=10^{-9}$ and $warmup\_step=2000$. This setup varies the learning rate of the model during training progress by increasing it linearly for the first 2000 training steps and decreasing it after that proportionally to the inverse square root of the step number. For other models, we use the standard Adam optimizer with a fixed learning rate of 0.001 in training.

We configure the training progress with a batch size of 8 in 30 epochs on an NVIDIA Tesla P100 GPU via the Kaggle platform\footnote{\url{https://www.kaggle.com/}}.
% We train each model in turn on each specific number of answers used per question during the training and evaluation. 
After each epoch, the performance loss on the train and development sets is calculated using the Cross-Entropy Loss function. The maximum length of the model-generated output is limited to 500 tokens to reduce the generating time of repetitive loops caused by text degeneration.


==> old/sections/5-results1.tex <==
\section{Experimental Results}
% \subsection{Overall Results}
% \begin{table*}[ht]
% \setlength{\tabcolsep}{4pt}
% %\renewcommand{\arraystretch}{1}
% \centering
% \begin{tabular}{l|l|ccccc}
% \toprule
% \multicolumn{2}{c}{{\color[HTML]{000000} \textbf{Model}}} &
%   {\color[HTML]{000000} \textbf{Max. \# responses}} &
%   {\color[HTML]{000000} \textbf{BLEU-1}} &
%   {\color[HTML]{000000} \textbf{BLEU-4}} &
%   {\color[HTML]{000000} \textbf{METEOR}} &
%   {\color[HTML]{000000} \textbf{ROUGE-L}} \\\midrule
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 1} &
%   {\color[HTML]{000000} 21.79} &
%   {\color[HTML]{000000} 10.29} &
%   {\color[HTML]{000000} 25.34} &
%   {\color[HTML]{000000} 32.36} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 2} &
%   {\color[HTML]{000000} \textbf{\underline{26.62}}} &
%   {\color[HTML]{000000} \textbf{12.86}} &
%   {\color[HTML]{000000} 25.15} &
%   {\color[HTML]{000000} 33.66} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 3} &
%   {\color[HTML]{000000} 26.09} &
%   {\color[HTML]{000000} 12.63} &
%   {\color[HTML]{000000} \textbf{\underline{25.98}}} &
%   {\color[HTML]{000000} \textbf{33.68}} \\
% \multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} RNN-1 \cite{bahdanau2016neural}}}} &
%   {\color[HTML]{000000} 4} &
%   {\color[HTML]{000000} 24.48} &
%   {\color[HTML]{000000} 11.55} &
%   {\color[HTML]{000000} 23.79} &
%   {\color[HTML]{000000} 31.92} \\\midrule
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 1} &
%   {\color[HTML]{000000} 21.04} &
%   {\color[HTML]{000000} 10.94} &
%   {\color[HTML]{000000} \textbf{24.72}} &
%   {\color[HTML]{000000} \textbf{\underline{33.95}}} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 2} &
%   {\color[HTML]{000000} 24.07} &
%   {\color[HTML]{000000} 11.3} &
%   {\color[HTML]{000000} 23.81} &
%   {\color[HTML]{000000} 31.92} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 3} &
%   {\color[HTML]{000000} 23.8} &
%   {\color[HTML]{000000} 10.95} &
%   {\color[HTML]{000000} 23.65} &
%   {\color[HTML]{000000} 31.65} \\
% \multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} RNN-2 \cite{luong-etal-2015-effective}}}} &
%   {\color[HTML]{000000} 4} &
%   {\color[HTML]{000000} \textbf{24.62}} &
%   {\color[HTML]{000000} \textbf{11.64}} &
%   {\color[HTML]{000000} 24.16} &
%   {\color[HTML]{000000} 31.97} \\\midrule

% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 1} &
%   {\color[HTML]{000000} 19.17} &
%   {\color[HTML]{000000} 9.51} &
%   {\color[HTML]{000000} \textbf{22.76}} &
%   {\color[HTML]{000000} \textbf{32.29}} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 2} &
%   {\color[HTML]{000000} 21.63} &
%   {\color[HTML]{000000} \textbf{10.81}} &
%   {\color[HTML]{000000} 20.66} &
%   {\color[HTML]{000000} 30.71} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 3} &
%   {\color[HTML]{000000} 22.08} &
%   {\color[HTML]{000000} 10.68} &
%   {\color[HTML]{000000} 20.96} &
%   {\color[HTML]{000000} 30.84} \\
% \multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} Convolutional \cite{10.5555/3305381.3305510}}}} &
%   {\color[HTML]{000000} 4} &
%   {\color[HTML]{000000} \textbf{22.16}} &
%   {\color[HTML]{000000} 10.32} &
%   {\color[HTML]{000000} 19.85} &
%   {\color[HTML]{000000} 29.49} \\\midrule
 
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 1} &
%   {\color[HTML]{000000} 21.84} &
%   {\color[HTML]{000000} 10.82} &
%   {\color[HTML]{000000} 23.37} &
%   {\color[HTML]{000000} 31.67} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 2} &
%   {\color[HTML]{000000} 24.81} &
%   {\color[HTML]{000000} 13.22} &
%   {\color[HTML]{000000} 24.6} &
%   {\color[HTML]{000000} 32.25} \\
% \multicolumn{2}{l}{{\color[HTML]{000000} }} &
%   {\color[HTML]{000000} 3} &
%   {\color[HTML]{000000} 24.9} &
%   {\color[HTML]{000000} 13.64} &
%   {\color[HTML]{000000} 21.72} &
%   {\color[HTML]{000000} 32.2} \\
% \multicolumn{2}{l}{\multirow{-4}{*}{{\color[HTML]{000000} Transformer \cite{NIPS2017_3f5ee243}}}} &
%   {\color[HTML]{000000} 4} &
%   {\color[HTML]{000000} \textbf{25.65}} &
%   {\color[HTML]{000000} \textbf{\underline{14.93}}} &
%   {\color[HTML]{000000} \textbf{24.85}} &
%   {\color[HTML]{000000} \textbf{33.05}} \\\midrule

% \end{tabular}
% \caption{Performances of baseline models on each experiment condition in the test set of ViCovidQA}
% \label{tbl_overall_results}
% \end{table*}

Table \ref{tbl_overall_results} presents the performance of our baseline models on different settings of the ViCovidQA dataset. The final score of each metric in the table is achieved by calculating the average scores of all model-generated answers.

Evaluated using BLEU-1 and BLEU-4, the performance of models tends to improve when applying more paraphrased answers in the experiments,
though this trend behaves differently among models.
RNN-1 using two answers per question achieved the
best BLEU-1 of 26.62\% while on BLEU-4, Transformer using four answers outperforms other models
with a score of 14.38\%. Apart from RNN-1 achieves
best score when applying two answers, other models
have highest performance when training and evaluating using four answers.


% It illustrate diverse results of model performances based on different metrics and number of responses used during the experiments.
% Table \ref{tbl_overall_results} presents the performance of our baseline models on each number of answers used per question in the test set of ViCovidQA. The final score of each metric in the table is achieved by calculating the average scores of all model-generated answers.

In contrast with the BLEU score, the performance of models evaluated by METEOR and ROUGE-L varies significantly under different dataset settings. As shown in the table, RNN-2 and Convolutional perform well when using only one response, with scores of 33.95\% and 32.29\% respectively, while RNN-1 and Transformer need to apply more answers to achieve better scores.

% It can be assumed that using multiple paraphrased answers has significantly influenced the performance of Transformer. The model itself tends to have better generalization reflected in all metrics when we increase the number of answers used in the experiments. Interestingly, the best performance of Transformer on four evaluation metrics are all achieved when applying all four paraphrased answers.


% For RNN model with Bahdanau attention, achieved best result using two answer at most on BLEU-1 and BLEU-4, best METEOR and ROUG-L achieved using at most 3 answers.

% For RNN model with Luong attention, best BLEU-1 and BLEU-4 is achieved using maximum 4 answers. Best BLEU-1 and BLEU-4 is achieved using one answers.
% The performance results of baseline models are presented in Table 3.

\subsection{Error Analysis}

%v1.0
% \begin{table*}[ht]
% \begin{center}
% \begin{tabular}{p{0.95\linewidth}}
% \hline \textbf{\underline{Question:}} Ưu điểm và nhược điểm của xét nghiệm kháng nguyên? (\textbf{English:} Advantages and disadvantages of antigen testing?)\\

% \textbf{\underline{Answer:}} -Ưu điểm: Có thể tiến hành trong thời gian ngắn. Chi phí rẻ. Có thể sản xuất hàng loạt đảm bảo đáp ứng nhu cầu. Phù hợp sử dụng đầu tiên để khoanh vùng dịch trên diện rộng.
% -Nhược điểm: Độ chính xác không cao. (\textbf{English:} -Pros: It can be done in a short time. Cheap cost. It is possible to mass produce to ensure that demand is met. Suitable for the first use for wide-ranging zoning. -Cons: The accuracy is not high.\\

% \textbf{\underline{Generated answer}}:
% theo quy định tại điều 2 nghị định số 21 quyết định số 23/2021 / qđ-ttg và các điều kiện hưởng lương từ ngày 07/7/2021 của thủ tướng chính phủ quy định tại điều 1 quyết định số 23/2021 / qđ-ttg và điều kiện hưởng lương từ ngày 07/7/2021 của thủ tướng chính phủ quy định tại điều 1 quyết định số 23/2021 / qđ-ttg ngày qđ-ttg ngày qđ-ttg ngày qđ-ttg ngày 01 năm 2020 / qđ-ttg ngày 01 năm 2020 / qđ-ttg ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 đến ngày 01 năm 2020 ... (\textbf{English:} according to the provisions of Article 2 of Decree No. 21 of Decision No. 23/2021/qd-ttg and salary conditions
% from 7/7/2021 of the Prime Minister specified in Article 1 of Decision No. 23/2021/qd-ttg and Article 1.
% conditions for receiving salary from 7/7/2021 of the Prime Minister specified in Article 1 of Decision No. 23/2021
% / qd-ttg date qd-ttg date qd-ttg date qd-ttg date 01, 2020 / qd-ttg date 01, 2020 / qd-ttg date
% 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 to 01, 2020 ...)
% \\\hline
% \textbf{\underline{Question:}} Các loại vắc-xin có hiệu quả chống lại biến thể Delta không? (\textbf{English:} Are the vaccines effective against the Delta variant?)\\

% \textbf{\underline{Answer:}} Tiến sĩ nói rằng vắc-xin COVID-19 có khả năng bảo vệ kém hơn bao nhiêu đối với Delta trong thế giới thực tại thời điểm này. Ông nói: “Ngay cả khi biến thể này có thể tránh được tác dụng của vắc-xin, thì càng có nhiều người được tiêm vắc-xin, dịch bệnh càng ít có khả năng lây lan”.
% Các báo cáo cho thấy hai liều vắc-xin Pfizer-BioNTech cung cấp khả năng bảo vệ 79\% chống lại nhiễm trùng biến thể delta. Nó dường như có hiệu quả 88\% đối với các triệu chứng nếu bị nhiễm bệnh.
% Hai liều vắc-xin AstraZeneca có 92\% thành công trong việc ngừng nhập viện do biến thể delta. (\textbf{English:} Dr. says how much less protection the COVID-19 vaccine has for Delta in the real world at the moment. "Even if this variant can avoid the effects of the vaccine, the more people are vaccinated, the less likely the disease is to spread," he said. Reports suggest that two doses of the Pfizer-BioNTech vaccine provide 79\% protection against delta variant infections.It appears to be 88\% effective for symptoms if infected.Two doses of AstraZeneca vaccine had a 92\% success in stopping hospital admissions due to delta variant.)\\

% \textbf{\underline{Generated Answer:}} biến thể delta không có tác dụng phụ (\textbf{English:} delta variant has no side effects)\\\hline

% \end{tabular}
% \end{center}
% \caption{Examples of incorrect generated answer}
% \label{tbl_error_analysis} 
% \end{table*}



% \begin{table*}[ht]
% \begin{center}
% \begin{tabular}{p{0.95\linewidth}}
% \hline 
% \textbf{\underline{Question:}} Tôi bị viêm mũi dị ứng đang uống thuốc có thể chích ngừa vaccine Covid-19 được không? Tôi không bị tiểu đường, huyết áp ổn định đo thường 116/65. (Can I get the Covid-19 vaccine if I have allergic rhinitis and am taking medication? I don't have diabetes, my blood pressure is stable at 116/65.)\\

% \textbf{\underline{Original Answer:}} Chào chị , tình trạng viêm mũi dị ứng đang dùng thuốc, chị nên trì hoãn tiêm vaccine Covid-19 đến khi bệnh được điều trị ổn định. Cảm ơn câu hỏi của chị. Trân trọng! (Hello madam, with the condition of allergic rhinitis on medication, you should delay the Covid-19 vaccine until the disease is treated stably. Thank you for your question. Best regards!)\\

% \textbf{\underline{Generated Answer:}} chào anh / chị , nếu bệnh tiểu đường của anh / chị đã ổn định , anh / chị có thể tiêm vaccine covid-19 . tuy nhiên , anh / chị nên tiêm tại bệnh viện hoặc cơ sở y tế có đủ năng lực hồi sức cấp cứu ban đầu . cảm ơn câu hỏi của anh / chị . trân trọng ! (hello sir / madam, if your diabetes is stable, you can get the covid-19 vaccine. however , you should give the injection at a hospital or medical facility that has the capacity to provide first aid . thank you for your question . best regards)\\\hline

% \textbf{\underline{Question:}} Tôi bị viêm gan B mạn tính thể hoạt động, đang uống thuốc điều trị tháng thứ 33. Theo kết quả xét nghiệm gần nhất vào tháng 4/2021, các chỉ số về men gan bình thường, chỉ số HBeAg ban đầu là dương tính đã chuyển âm tính từ tháng 9/2020, đo lượng virus dưới ngưỡng phát hiện. Vậy xin hỏi bác sĩ tôi có thể thực hiện tiêm vaccine Covid-19 được không? (I have active chronic hepatitis B, I am taking medication for the 33rd month. According to the most recent test results in April 2021, indicators of liver enzymes were at normal levels, the initial HBeAg index has turned from positive to negative since September 2020, measuring the amount of virus below the detection threshold. Can I get the Covid-19 vaccine?)\\

% \textbf{\underline{Original Answer:}} Nếu các bệnh lý mãn tính đã ổn định trong vòng 3 tháng trước khi tiêm chủng (có nghĩa là bệnh không cần thay đổi điều trị đáng kể hoặc nhập viện vì bệnh lý nặng hơn), các chỉ số xét nghiệm duy trì ở mức độ ổn, anh hoàn toàn có thể tiêm được vaccine phòng Covid-19.(If chronic pathologies have stabilized within 3 months before vaccination (the disease does not require significant treatment changes or is forced to be hospitalized due to a more severe pathology), the test indicators remain at a stable level, you can get the vaccine against Covid-19.)\\

% \textbf{\underline{Generated answer}}: chào anh , nếu tình trạng bệnh lý của anh / chị đã ổn định , các chỉ số về mạch , huyết áp , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , nhịp thở , ... , nhịp thở , nhịp thở , các chỉ số xét nghiệm duy trì ở mức độ ổn , anh hoàn toàn có thể tiêm được vaccine covid-19 . cảm ơn câu hỏi của anh / chị . trân trọng ! (hello sir , if your medical condition has stabilized , indicators of pulse , blood pressure , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , breathing rate , ... , breathing rate , breathing rate , the test indicators remain at a stable level , you can fully vaccinate covid-19 . Thank you for your question . best regards !)\\\hline
% \end{tabular}
% \end{center}
% \caption{Examples of generated answers that contain errors}
% \label{tbl_error_analysis} 
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% After the experiments on ViCovidQA, we analyze the evaluation results to identify the errors and gain more in-depth insights into model performances. Through this analysis process, various mistakes and errors have been pointed out in the generated answers of all models. In summary, these errors are divided into three main groups. Table \ref{tbl_error_analysis} describes examples of generated answers that have errors. 

% \begin{itemize}
%     \item The first group includes meaningless and illogical answers. In some cases, the generated answers are just a set of tokens arranged in a chaotic order. This means that the model is underfitting and should be trained on larger data or increase its complexity. 
    
%     \item The second group contains meaningful and coherent answers but do not satisfy the question's requirements. As seen from the first example in the table, the question asks the possibility of getting COVID-19 vaccine while taking allergic rhinitis medication and not having diabetes. The original answer suggests the person delay the vaccine until the condition is stable, but the generated one assumes that the person has only diabetes and can get the vaccine if the condition is stable. This type of error can be caused by the diverse Vietnamese vocabulary and grammar, which makes the model difficult to understand the context of question.
    
%     \item The third group consists of text degeneration. Typically, this is a common phenomenon in sequence-to-sequence learning tasks when a word or a phrase is infinitely repeated in the generated sequence. In the second example in the table, the generated answer seems to match the question at the beginning when it mentions "nếu tình trạng bệnh lý của anh / chị đã ổn định" (if your medical condition has stabilized), but after that text degeneration appears when the word "nhịp thở" (breathing rate) is repeatedly generated.
% \end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


From the experiment results, we determine that the Transformer trained on four answers gives the best performance among others based on BLEU-4 according to the approach of \newcite{kacupaj2021paraqa}. Twenty samples are randomly chosen from the generated answers of the model to perform error analysis. We calculate the average length and vocabulary size and count the number of POS tags in the references and generated answers. The statistics of the analysis process are shown in Table \ref{tbl_stat_analysis}.

\begin{table}[H]
    \renewcommand{\arraystretch}{1.2}
    \small
    \begin{tabular}{p{2.3cm}p{2.7cm}p{1.6cm}}\hline
     & \textbf{Original answers}  &  \textbf{Generated answers} \\\hline
     Avg. length  & \multicolumn{1}{r}{115.53}  & \multicolumn{1}{r}{75.25} \\
     Vocabulary size  & \multicolumn{1}{r}{776}  & \multicolumn{1}{r}{114}  \\
     \# POS tag  & \multicolumn{1}{r}{16}  & \multicolumn{1}{r}{12}\\\hline
    \end{tabular}
    \caption{The average length, vocabulary size and number of POS tag in 20 generated samples and their references}
    \label{tbl_stat_analysis} 
\end{table}


The vocabulary size of the output answers is almost seven times less than that of the original answers, while the average length and number of POS tags do not vary significantly. This implies that Transformer does not generalize well, and the tokens overlapping or text degeneration may have occurred in the outputs of the model.

By checking the generated result, we notice some output answers contain overlapping phrases and do not match the question and reference answers. Two samples of the generated answers are presented in Table \ref{tbl_error_analysis}. As shown in the table, the two generated answers are quite similar in meaning regardless of the difference between the two questions. Moreover, the phrase "10.000.000 đồng" (VND 10.000.000) keeps repeated in both examples.

\begin{table*}[!ht]
\renewcommand{\arraystretch}{1.2}
\begin{center}
\begin{tabular}{p{0.95\linewidth}}
\hline 
\textbf{\underline{Question:}} Trẻ sơ sinh nhiễm COVID-19 qua đường nào ? [\textbf{English: }By which way do babies get COVID-19?]\vspace{0.3em}\\

\textbf{\underline{Original Answer:}} - trẻ sơ sinh nhiễm sars-cov-2 theo 3 cách : lây trong tử cung ( qua đường máu hoặc nước ối từ mẹ nhiễm sars-cov-2 ) ; lây trong cuộc đẻ ( tiếp xúc dịch tiết mẹ như máu , dịch ối) và lây sau đẻ ( qua tiếp xúc với mẹ hay người chăm sóc sau sinh ) ; các dữ liệu khoa học đến nay chưa kết luận đường lây qua sữa mẹ . trong đó lây nhiễm trước và trong sinh ít khi xảy ra , chủ yếu lây nhiễm trong quá trình chăm sóc sau sinh . [\textbf{English: }Infants infected with sars-cov-2 in three ways: intrauterine infection (via blood or amniotic fluid from the mother infected with sars-cov-2) ; transmission during childbirth (exposure to maternal secretions such as blood, amniotic fluid) and postpartum transmission (through contact with the mother or postpartum caregiver); the scientific data has not concluded the route of transmission through breast milk. in which infection before and during childbirth rarely occurs, mainly infectious during postpartum care]\\

\textbf{\underline{Generated Answer:}} theo quy định tại điều 11 nghị định số 176 / 2013 / nđ-cp ngày 14/11/2013 của chính phủ về xử phạt hành chính trong lĩnh vực y tế , hành vi không bị phạt tiền từ 5.000.000 đồng đến 10.000.000 đồng đến 10.000.000 đồng đến 10.000.000 đồng đến ... [\textbf{English: }In accordance with Article 11 of the Government's Decree No. 176/2013/nd-cp dated November 14, 2013 on administrative sanctions in the health sector, acts not subject to a fine of from VND 5,000,000 to VND 10,000,000 to VND 10,000,000 to VND 10,000,000 ...]\\\hline

\textbf{\underline{Question:}} Biến chủng Epsilon ( B. 1.427 / B. 1.429 ) là gì ? [\textbf{English: }What is epsilon (B. 1,427/B. 1,429) variant?]\\

\textbf{\underline{Original Answer:}} biến chủng này có thể tự sắp xếp lại một phần của protein đột biến mà virus sử dụng để liên kết với các tế bào của cơ thể . vì thế , biến chủng epsilon có khả năng lây nhiễm cao hơn khoảng 20 \% và dễ dàng làm suy yếu hệ miễn dịch của con người . [\textbf{English: }This variant can rearrange a portion of the mutated protein that the virus uses to bind to the body's cells. Therefore, epsilon variants are about 20\% more contagious and easily weaken the human immune system.]\\

\textbf{\underline{Generated Answer:}} theo quy định tại điều 11 nghị định số 176 / 2013 / nđ-cp ngày 14/11/2013 của chính phủ về xử phạt hành chính trong lĩnh vực y tế , hành vi không thực hiện biện pháp cách ly y tế tại điều 11 nghị định số 176 / 2013 / nđ-cp ngày 14/11/2013 của chính phủ về xử phạt hành chính trong lĩnh vực y tế , hành vi có hành vi có hành vi này bị phạt tiền từ 5.000.000 đồng đến 10.000.000 đồng đến 10.000.000 đồng đến 10.000.000 đồng ... [\textbf{English: }In accordance with Article 11 of the Government's Decree No. 176/2013/nd-cp dated November 14, 2013 on administrative sanctions in the health sector, failure to implement medical isolation measures in Article 11 of the Government's Decree No. 176/2013/nd-cp dated November 14, 2013 on administrative sanctions in the health sector, acts committed in this act are subject to a fine of from VND 5,000,000,000 to VND 10,000,000 to VND 10,000,000 to VND 10,000,000 ...]\\\hline
\end{tabular}
\end{center}
\caption{Examples of answers generated by Transformer model that contain text degeneration}
\label{tbl_error_analysis} 
\end{table*}

Continuing by checking the result of other models, various mistakes and errors have been pointed out in the generated answers. In summary, these errors can be divided into three main groups.

\begin{itemize}
    \item The first group includes meaningless and illogical answers. In some cases, the generated answers are just a set of tokens arranged in a chaotic order.
    
    \item The second group contains meaningful and coherent answers but do not satisfy the question's requirements. This type of error can be caused by the diverse Vietnamese vocabulary and grammar, which makes the model difficult to understand the context of question.
    
    \item The third group consists of text degeneration. Typically, this is a common phenomenon in sequence-to-sequence learning tasks when a word or a phrase is infinitely repeated in the generated sequence indicating that the models may not generalize well.
\end{itemize}

% Table 5 shows the statisics of the average length, vocabulary size and number of POS tag .

% The statistical comparison between the original and generated answers are shown in the 

% We notice that, in some sentences, BLEU-1 score very low bu high BLEU-4 due to text degeneration.

% We also compare the generated answers between Transformer and convolutional network trained on 4 answers.



==> old/sections/6-conclusion1.tex <==
\section{Conclusion and Future Works}
In this paper, we introduced ViCovidQA, the first community-based question answering dataset about COVID-19 for Vietnamese. Our dataset comprises 4,500 question-answer pairs with multiple paraphrased answers. We evaluated the dataset's quality through various baseline deep learning models and commonly used metrics such as BLEU, METEOR, and ROUGE-L. 

We illustrated the effect of having multiple paraphrased answers for experiments with baseline models and provided benchmark results for further research. 
% RNN with Bahdanau attention using two answers gives the best BLEU-1 of 26.62\% and gives the best METEOR of 25.98\% when applying three answers.
RNN with Bahdanau attention achieves the best BLEU-1 and METEOR scores of 26.62\% and 25.98\% when applying two and three answers respectively. 
Transformers using four answers outperforms others on BLEU-4 with score of 14.38\%. On ROUGE-L, RNN with Luong Attention using one answer has the best performance of 33.95\%. The advantage of having multiple paraphrased answers is greatly illustrated by BLEU scores, on which three out of four models achieve the highest performance when applying all four paraphrased answers. On the contrary, our experiments showed that METEOR and ROUGE-L scores do not give a clear reflection of the improvement in models performance when increase number of answer used.

Generally, the performance of these models is not quite good since the generated answers contain various errors. There are several reasons for this: the diversity of the Vietnamese language, lacking a specific evaluation metric for the Vietnamese language, the long-sequence content, and the size limitation of our dataset. The dataset offers a valuable contribution to the community, providing the foundation for many research lines in the single-turn QA domain and other areas. 

In the future, we will expand ViCovidQA by collecting more relevant question-answer pairs and creating more paraphrased answers. We will also investigate replacing the embedding layer with pre-trained word embeddings for Vietnamese, such as PhoBert \cite{phobert} to improve model performance.


